Comicolorization: Semi-Automatic Manga Colorization

We developed "Comicolorization", a semi-automatic colorization system for manga images. Given a monochrome manga and reference images as inputs, our system generates a plausible color version of the manga. This is the first work to address the colorization of an entire manga title (a set of manga pages). Our method colorizes a whole page (not a single panel) semi-automatically, with the same color for the same character across multiple panels. To colorize the target character by the color from the reference image, we extract a color feature from the reference and feed it to the colorization network to help the colorization. Our approach employs adversarial loss to encourage the effect of the color features. Optionally, our tool allows users to revise the colorization result interactively. By feeding the color features to our deep colorization network, we accomplish colorization of the entire manga using the desired colors for each panel.

==> Makefile <==
# make -f Makefile_latex

R ?= comicolorization_arxiv
STY = *.cls
FIG = images/samplefigure.pdf

pdf: $(R).pdf

$(R).pdf:
	pdflatex $(R).tex
	bibtex $(R)
	pdflatex $(R).tex

buildarxiv: ms.pdf

ms.pdf:
	mv comicolorization_arxiv.tex ms.tex || true
	pdflatex ms.tex
	bibtex ms
	pdflatex ms.tex
	bibtex ms
	pdflatex ms.tex

cleanarxiv: ms.pdf
	rm -rf */*.py */*.ipynb **/*.md  acmart.bib *.log *.dvi *.ps *.out \
	images/drawn_page_first5 images/objective_evaluation images/oldfig \
	comicolorization_arxiv_v* comicolorization_tb* comicolorization_SA* comicolorization_arxiv.pdf \
	supplementarymaterials* *~

FILE = comicolorization_arxiv
tbmain: $(FILE).tex
		platex $(FILE)
		platex $(FILE)
		bibtex $(FILE)
		bibtex $(FILE)
		platex $(FILE)
		platex $(FILE)
		dvipdfmx $(FILE).dvi

S_FILE = supplementarymaterials
tbsupply: $(S_FILE).tex
	platex $(S_FILE)
	platex $(S_FILE)
	bibtex $(S_FILE)
	bibtex $(S_FILE)
	platex $(S_FILE)
	platex $(S_FILE)
	dvipdfmx $(S_FILE).dvi

clean:
	rm -rf *.log *.dvi *.out *.aux *.bbl *.blg

